TPMCF: Temporal QoS Prediction using Multi-Source Collaborative Features

Recently, with the rapid deployment of service APIs, personalized service recommendations have played a paramount role in the growth of the e-commerce industry. Quality-of-Service (QoS) parameters determining the service performance, often used for recommendation, fluctuate over time. Thus, the QoS prediction is essential to identify a suitable service among functionally equivalent services over time. The contemporary temporal QoS prediction methods hardly achieved the desired accuracy due to various limitations, such as the inability to handle data sparsity and outliers and capture higher-order temporal relationships among user-service interactions. Even though some recent recurrent neural-network-based architectures can model temporal relationships among QoS data, prediction accuracy degrades due to the absence of other features (e.g., collaborative features) to comprehend the relationship among the user-service interactions. This paper addresses the above challenges and proposes a scalable strategy for Temporal QoS Prediction using Multi-source Collaborative-Features (TPMCF), achieving high prediction accuracy and faster responsiveness. TPMCF combines the collaborative-features of users/services by exploiting user-service relationship with the spatio-temporal auto-extracted features by employing graph convolution and transformer encoder with multi-head self-attention. We validated our proposed method on WS-DREAM-2 datasets. Extensive experiments showed TPMCF outperformed major state-of-the-art approaches regarding prediction accuracy while ensuring high scalability and reasonably faster responsiveness.

==> components/0_abstract.tex <==
\begin{abstract}
In recent times, with the proliferation of online activities and the rapid deployment of web service APIs, personalized service recommendations have played a paramount role in the growth of the e-commerce industry. The performance of web services is one of the standard measures for service recommendation. Quality-of-Service (QoS) parameters determining the service performance fluctuate over time for a user. Thus, for a given user, the service QoS prediction over time plays an essential part in identifying a suitable service to invoke among a pool of services having the same functionality. 
The contemporary temporal QoS prediction methods hardly achieved the desired accuracy due to various limitations, such as data sparsity, the presence of outliers, and the inability to capture higher-order temporal relationships among user-service interactions. Even though some recent recurrent neural network-based sequential architectures can model temporal relationships among QoS data, the prediction accuracy degrades due to the absence of other features (e.g., collaborative self features, collaborative spatial features of users/services) to capture the relationship among the user-service interactions. In addition to the lack of effective representation of implicit features, having the same attention across all the features in every timestep may impede improving the prediction accuracy.
% 
% The contemporary temporal QoS prediction methods hardly achieved the desired accuracy due to various limitations, such as data sparsity, the presence of outliers, and the inability to capture higher-order temporal relationships among user-service interactions. 
% Even though some recent recurrent neural network-based sequential architectures can model temporal relationships among QoS data, the prediction accuracy degrades due to the absence of other features (e.g., collaborative self features, collaborative spacial features of users/services) to capture relationship among the user-service interactions. 
% Even though some recent recurrent neural network-based sequential architectures can model temporal relationships among QoS data, the absence of other features (e.g., collaborative self features, collaborative spacial features of users/services) to capture relationship among the user-service interactions may cause accuracy degradation on QoS prediction. 
% On the one hand, (a) the lack of effective representation of implicit features; (b) the lack of having different attention provides on the temporal 
% 
This paper addresses the above challenges and proposes a scalable strategy for {\textbf{T}}emporal QoS {\textbf{P}}rediction using {\textbf{M}}ulti-source {\textbf{C}}ollaborative {\textbf{F}}eatures (namely, TPMCF) enabling faster responsiveness while attaining high prediction accuracy. 
Our work combines the collaborative features of the user/service by exploiting the user-service relationship with the spatio-temporal auto-extracted features by employing graph convolution and a variant of transformer encoder with multi-head self-attention. 
% Our work uses spatio-temporal auto-extracted features along with collaborative features for the users/services to capture complex relationships among QoS data employing graph convolution matrix factorization and adaptive transformer encoder with multi-head self-attention. 
While the graph convolutional is responsible for automatic feature extraction exploiting the spatial information, the transformer encoder is accountable for capturing the temporal dependency among QoS data for prediction. We validated our proposed method on WS-DREAM-2 benchmark dataset. Extensive experiments showed that TPMCF outperformed the major state-of-the-art approaches in terms of prediction accuracy while ensuring high scalability and reasonably faster responsiveness.
\end{abstract}


% Quality-of-Service (QoS) parameters deciding the performance of services fluctuate over time for a user. Therefore, the QoS prediction of services over time for a user is crucial to determine a suitable service to invoke among services with the same functionality. The traditional temporal QoS prediction methods hardly achieve the desired accuracy due to various limitations, such as data sparsity, the presence of outliers, and the inability to capture temporal relationships among user-service interactions. Even though some recent recurrent neural network-based sequential architectures can model temporal relationships among QoS data, the use of handcrafted features results in accuracy degradation on service QoS prediction due to a lack of effective representation of implicit features. In this paper, we address these challenges and propose a highly scalable strategy for temporal QoS prediction enabling faster responsiveness with high prediction accuracy. Our work utilizes spatio-temporal features to capture complex relationships among QoS data employing graph convolution and multi-head self-attention networks. While the graph convolutional network is accountable for automatic feature generation exploiting the spatial information, the multi-head self-attention network utilizes temporal features for QoS prediction. We validate our proposed method on WS-DREAM-2 benchmark dataset. Our extensive experiments showed that our framework outperformed the major state-of-the-art approaches in terms of prediction time and accuracy.

